Stability of Axion--SU(2) Chromomagnetic Condensates with Stochastic Spin-2 Dressing

We investigate whether a stochastic spin-2 gauge-field background can stabilize the chromomagnetic condensate of axion--SU(2) Yang--Mills theory at fixed axion Noether charge in flat spacetime. By coarse-graining the gauge field, we uncover a new class of statistically homogeneous and isotropic spin-2-dressed chromomagnetic condensates satisfying the classical background equations. We then study their fluctuations in two steps. First, at the mean-field (Hartree) level, we determine the fluctuation spectrum and the region where all modes remain positively gapped. Second, we include the leading scattering corrections from fluctuations propagating through the stochastic background. We find that gap survival is controlled by non-Gaussian correlations of the dressing. Statistical positivity constrains the otherwise undetermined higher-point contributions through model-independent consistency conditions, without fixing their detailed momentum dependence. These bounds separate the Hartree-gapped region into a part where a positive Born-level gap is ruled out and a part where stability remains possible. The results are relevant to non-Abelian gauge condensates in early-universe cosmology, including inflation, dark energy, and primordial gravitational waves, and to QCD-like gauge sectors above confinement where thermal effects are subleading.

==> linear_W_vertex_equation_macros.tex <==
% Load this file in the preamble of your manuscript.
% The diagram is then inserted with \LWVertexEquation.
\RequirePackage{amsmath}
\RequirePackage{graphicx}
\RequirePackage{tikz}
\usetikzlibrary{decorations.pathmorphing,arrows.meta}

% Colours sampled from the supplied figures.
\definecolor{LWVquantum}{RGB}{174,75,244}
\definecolor{LWVdressing}{RGB}{28,108,104}
\definecolor{LWVeffective}{RGB}{60,180,255}
\definecolor{LWVcubic}{RGB}{43,108,192}
\definecolor{LWVquartic}{RGB}{234,153,142}
\definecolor{LWVaxion}{RGB}{174,53,44}

\tikzset{
  LWV/wave/.style={
    decorate,
    decoration={snake,amplitude=.43mm,segment length=2.35mm,
                pre length=.4mm,post length=.4mm},
    line width=.78pt
  },
  LWV/quantum/.style={LWV/wave,draw=LWVquantum},
  LWV/dressing/.style={LWV/wave,draw=LWVdressing},
  LWV/homogeneous/.style={LWV/wave,draw=LWVaxion},
  LWV/axion/.style={draw=LWVaxion,dashed,line width=.78pt},
  LWV/flow/.style={
    -{Stealth[length=1.25mm,width=.95mm]},line width=.48pt
  }
}

% Incoming and outgoing quantum fluctuation legs.
\newcommand{\LWVQuantumLegs}{%
  \draw[LWV/quantum] (-1.22,0)--(0,0);
  \draw[LWV/quantum] (0,0)--(1.22,0);
  \draw[LWV/flow] (-1.02,.23)--(-.63,.23);
  \draw[LWV/flow] (.63,.23)--(1.02,.23);
  \node[above,inner sep=1pt] at (-.825,.25) {$\mathbf p$};
  \node[above,inner sep=1pt] at (.825,.25) {$\mathbf k$};
  \node[below,text=LWVquantum,inner sep=1pt]
    at (-.97,-.12) {$\mathcal A_b^j$};
  \node[below,text=LWVquantum,inner sep=1pt]
    at (.97,-.12) {$\mathcal A_a^i$};
}

% Crossed-circle endpoint for a prescribed background field.
\newcommand{\LWVBackgroundEnd}[2]{%
  \begin{scope}[shift={(#1)}]
    \draw[draw=#2,line width=.67pt,fill=white] (0,0) circle (.052);
    \draw[draw=#2,line width=.60pt]
      (-.034,-.034)--(.034,.034)
      (-.034,.034)--(.034,-.034);
  \end{scope}
}

% The single diagrammatic equation: effective vertex = its three terms.
% All labels use phi, not alpha. No q_Q label is included.
\newcommand{\LWVertexEquation}{%
\begin{tikzpicture}[baseline=-.55ex,every node/.style={font=\small}]
  % (1): effective three-leg kernel.
  \begin{scope}
    \LWVQuantumLegs
    \draw[LWV/dressing] (0,1.23)--(0,0);
    \LWVBackgroundEnd{0,1.28}{LWVdressing}
    \node[above,text=LWVdressing] at (0,1.39)
      {$W_\lambda(\mathbf q)$};
    \fill[LWVeffective] (0,0) circle (.115);
    \node at (0,-.77)
      {$g\,[\mathcal V_\lambda(\mathbf q;\mathbf p)]^{ij}_{ab}$};
  \end{scope}

  \node[font=\large] at (1.825,0) {$=$};

  % (3), first term: cubic Yang--Mills derivative vertex.
  \begin{scope}[shift={(3.65,0)}]
    \LWVQuantumLegs
    \draw[LWV/dressing] (0,1.23)--(0,0);
    \LWVBackgroundEnd{0,1.28}{LWVdressing}
    \node[above,text=LWVdressing] at (0,1.39)
      {$W_\lambda(\mathbf q)$};
    \fill[LWVcubic] (0,0) circle (.064);
    % Small open circle: derivative coupling, as in the supplied legend.
    \draw[draw=LWVcubic,fill=white,line width=.67pt]
      (.14,.18) circle (.049);
    \node at (0,-.77) {$g$};
  \end{scope}

  \node[font=\large] at (5.475,0) {$+$};

  % (3), second term: quartic Yang--Mills vertex with Q insertion.
  \begin{scope}[shift={(7.30,0)}]
    \LWVQuantumLegs
    \draw[LWV/dressing] (-.69,1.235)--(0,0);
    \LWVBackgroundEnd{-.72,1.28}{LWVdressing}
    \node[above,text=LWVdressing] at (-.72,1.39)
      {$W_\lambda(\mathbf q)$};
    \draw[LWV/homogeneous] (.69,1.235)--(0,0);
    \LWVBackgroundEnd{.72,1.28}{LWVaxion}
    \node[above,text=LWVaxion] at (.72,1.39)
      {$Q\delta_i^{\,a}$};
    \fill[LWVquartic] (0,0) circle (.073);
    \node at (0,-.77) {$g^2$};
  \end{scope}

  \node[font=\large] at (9.125,0) {$+$};

  % (3), third term: axion Chern--Simons vertex.
  \begin{scope}[shift={(10.95,0)}]
    \LWVQuantumLegs
    \draw[LWV/dressing] (-.69,1.235)--(0,0);
    \LWVBackgroundEnd{-.72,1.28}{LWVdressing}
    \node[above,text=LWVdressing] at (-.72,1.39)
      {$W_\lambda(\mathbf q)$};
    \draw[LWV/axion] (.69,1.235)--(0,0);
    \LWVBackgroundEnd{.72,1.28}{LWVaxion}
    \node[above,text=LWVaxion] at (.72,1.39) {$\phi$};
    \fill[LWVaxion] (-.073,-.073) rectangle (.073,.073);
    \node at (0,-.77) {$g$};
  \end{scope}
\end{tikzpicture}%
}


==> su2_quadratic_preamble.tex <==
% Corrected SU(2) quadratic-action diagrams, 18 October 2026, version 3.
% Quadratic-action diagrams for SU(2) quantum fluctuations.
% Load before \begin{document}; compatible with the earlier tensor preamble.
% All names are prefixed QA to avoid collisions.
% Each action diagram means 1/2 int A Delta_r A, including its signed kernel.
% Coupling labels alone are not complete amputated Feynman rules.
% The background axion is rescaled as in the earlier figures: dot(phi)=alpha.
% For a canonical axion alpha=c_phi dot(phi), restore c_phi in CS labels.
% Momentum arrows show spatial momentum flow, never charge flow.
\RequirePackage{amsmath,amssymb,xcolor,tikz}
\usetikzlibrary{decorations.pathmorphing,calc,arrows.meta}

\definecolor{QAQuantum}{HTML}{AE4BF4}
\definecolor{QAW}{HTML}{1C6C68}
\definecolor{QAYM}{HTML}{2B6CC0}
\definecolor{QAQuartic}{HTML}{EA998E}
\definecolor{QABackground}{HTML}{AE352C}
\definecolor{QAInk}{HTML}{191E22}
\providecommand{\QADiagramScale}{1}

\tikzset{
  qa/quantum/.style={draw=QAQuantum,line width=1.0pt,decorate,
    decoration={snake,amplitude=1.05pt,segment length=5.8pt}},
  qa/tensor/.style={draw=QAW,line width=.95pt,decorate,
    decoration={snake,amplitude=1.05pt,segment length=5.8pt}},
  qa/qbackground/.style={draw=QABackground,line width=.95pt,decorate,
    decoration={snake,amplitude=1.05pt,segment length=5.8pt}},
  qa/axion/.style={draw=QABackground,line width=.9pt,
    dash pattern=on 3pt off 2.1pt},
  qa/ymvertex/.style={circle,fill=QAYM,draw=QAYM,
    inner sep=0pt,minimum size=6.0pt},
  qa/quarticvertex/.style={circle,fill=QAQuartic,draw=QAQuartic,
    inner sep=0pt,minimum size=6.0pt},
  qa/csvertex/.style={circle,fill=QABackground,draw=QABackground,
    inner sep=0pt,minimum size=6.4pt},
  qa/derivative/.style={circle,draw=QAYM,fill=white,line width=.9pt,
    inner sep=0pt,minimum size=5.2pt},
  qa/momentum/.style={font=\footnotesize,text=QAInk,inner sep=1pt},
  qa/weight/.style={font=\footnotesize,text=QAInk,inner sep=1pt},
  qa/flow/.style={draw=QAInk,line width=.5pt,
    -{Stealth[length=3.6pt,width=2.8pt]}}
}

\newcommand{\QABackgroundCross}[1]{%
  \draw[QABackground,line width=.8pt,fill=white] (#1) circle[radius=.105];
  \draw[QABackground,line width=.8pt]
    ($(#1)+(-.074,-.074)$)--($(#1)+(.074,.074)$);
  \draw[QABackground,line width=.8pt]
    ($(#1)+(-.074,.074)$)--($(#1)+(.074,-.074)$);
}
\newcommand{\QABeginVertex}{%
  \begin{tikzpicture}[x=.88cm,y=.82cm,scale=\QADiagramScale,
    transform shape,baseline=-.55ex]
  \path[use as bounding box] (-.12,-1.42) rectangle (3.83,1.27);
  \coordinate (v) at (1.50,0);
}
\newcommand{\QAEndVertex}{\end{tikzpicture}}
\newcommand{\QAIncoming}{%
  \draw[qa/quantum] (0,0)--(v);
  \draw[qa/flow] (.34,.22)--(1.02,.22);
  \node[qa/momentum,anchor=south] at (.68,.26) {$\mathbf k$};
}
\newcommand{\QAOutgoing}[1]{%
  \draw[qa/quantum] (v)--(2.51,-.88);
  \draw[qa/flow] (1.96,-.57)--(2.40,-.95);
  \node[qa/momentum,anchor=north] at (2.10,-1.00) {$#1$};
}
\newcommand{\QAUpperW}{%
  \draw[qa/tensor] (v)--(2.51,.88);
  \draw[qa/flow] (1.96,.57)--(2.40,.95);
  \node[qa/momentum,anchor=south] at (2.10,1.00) {$\mathbf p$};
  \node[qa/momentum,text=QAW,anchor=west] at (2.69,.88) {$W$};
}
\newcommand{\QAUpperQ}{%
  \coordinate (bqtop) at (2.51,.88);
  \draw[qa/qbackground] (v)--(bqtop);
  \QABackgroundCross{bqtop}
  \node[qa/momentum,text=QABackground,anchor=west] at (2.71,.88) {$Q$};
}
\newcommand{\QAUpperPhi}{%
  \coordinate (bphitop) at (2.51,.88);
  \draw[qa/axion] (v)--(bphitop);
  \QABackgroundCross{bphitop}
  \node[qa/momentum,text=QABackground,anchor=west] at (2.71,.88) {$\dot\phi$};
}
\newcommand{\QARightQ}{%
  \coordinate (bqright) at (3.08,0);
  \draw[qa/qbackground] (v)--(bqright);
  \QABackgroundCross{bqright}
  \node[qa/momentum,text=QABackground,anchor=west] at (3.28,0) {$Q$};
}
\newcommand{\QARightPhi}{%
  \coordinate (bphiright) at (3.08,0);
  \draw[qa/axion] (v)--(bphiright);
  \QABackgroundCross{bphiright}
  \node[qa/momentum,text=QABackground,anchor=west] at (3.28,0) {$\dot\phi$};
}
\newcommand{\QAVertexLabel}[1]{%
  \node[qa/weight,anchor=north east] at (1.39,-.16) {$#1$};
}
% Small open circle: a derivative in the quantum/background-field kernel.
% The time derivative already absorbed in the axion background is separate.
\newcommand{\QADerivativeMarker}[1][QAYM]{%
  \node[qa/derivative,draw=#1] at ($(v)+(-.10,.37)$) {};
}

% Homogeneous-background quadratic action.
\newcommand{\QADiagramKinetic}{%
  \QABeginVertex
  \draw[qa/quantum] (0,0)--(3.05,0);
  \draw[qa/flow] (1.175,.22)--(1.875,.22);
  \node[qa/momentum,anchor=south] at (1.525,.26) {$\mathbf k$};
  \node[qa/weight,anchor=north] at (1.525,-.18)
    {$\partial^\mu\partial_\mu$};
  \QAEndVertex
}
\newcommand{\QADiagramQDerivative}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k}\QAUpperQ
  \node[qa/ymvertex] at (v) {};
  \QADerivativeMarker
  \QAVertexLabel{g}
  \QAEndVertex
}
\newcommand{\QADiagramQQ}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k}\QAUpperQ\QARightQ
  \node[qa/quarticvertex] at (v) {};
  \QAVertexLabel{g^2}
  \QAEndVertex
}
\newcommand{\QADiagramPhiDerivative}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k}\QAUpperPhi
  \node[qa/csvertex] at (v) {};
  \QADerivativeMarker[QABackground]
  \QAEndVertex
}
\newcommand{\QADiagramQPhi}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k}\QAUpperQ\QARightPhi
  \node[qa/csvertex] at (v) {};
  \QAVertexLabel{g}
  \QAEndVertex
}

% W-dependent quadratic action: every vertex has TWO quantum A legs.
\newcommand{\QADiagramWDerivative}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k-\mathbf p}\QAUpperW
  \node[qa/ymvertex] at (v) {};
  \QADerivativeMarker
  \QAVertexLabel{g}
  \QAEndVertex
}
\newcommand{\QADiagramQW}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k-\mathbf p}\QAUpperW\QARightQ
  \node[qa/quarticvertex] at (v) {};
  \QAVertexLabel{g^2}
  \QAEndVertex
}
\newcommand{\QADiagramPhiW}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k-\mathbf p}\QAUpperW\QARightPhi
  \node[qa/csvertex] at (v) {};
  \QAVertexLabel{g}
  \QAEndVertex
}
\newcommand{\QADiagramWW}{%
  \QABeginVertex
  \QAIncoming\QAOutgoing{\mathbf k-\mathbf p-\mathbf q}\QAUpperW
  \draw[qa/tensor] (v)--(3.13,0);
  \draw[qa/flow] (2.33,.22)--(2.96,.22);
  \node[qa/momentum,anchor=south] at (2.65,.26) {$\mathbf q$};
  \node[qa/momentum,text=QAW,anchor=west] at (3.30,0) {$W$};
  \node[qa/quarticvertex] at (v) {};
  \QAVertexLabel{g^2}
  \QAEndVertex
}


% Quantum-field notation used in the main-text equation.
\newcommand{\QALegendQuantum}{%
  \tikz[baseline=-.45ex]{\draw[qa/quantum](0,0)--(.65,0);}}


==> tensor_diagram_preamble.tex <==
% Load this file in the preamble of your manuscript.
% Standalone, editable TikZ figure for stochastic tensor cross-spectra.
% Vertex labels indicate coupling dependence, not complete numerical kernels.
% Numerical and tensor factors retain the normalization of the displayed LHS.
% Momentum arrows indicate flow: k enters; p,q and the remainder leave.
% The trace-pair tadpole includes the single external stochastic contraction.
% The axion variable below is rescaled so that dot(phi) is the effective
% rolling-axion background previously denoted alpha (axion coupling absorbed).
% Ensemble averaging, integrations, helicity sums, and the common
% momentum delta function are implicit in the displayed products.
\RequirePackage{amsmath,amssymb}
\RequirePackage{xcolor}
\RequirePackage{tikz}
\usetikzlibrary{decorations.pathmorphing,calc,arrows.meta}

\definecolor{YMblue}{RGB}{43,108,192}
\definecolor{QuarticPink}{RGB}{234,153,142}
\definecolor{CSred}{RGB}{174,53,44}
\definecolor{Wgreen}{RGB}{28,108,104}
\definecolor{Ink}{RGB}{25,30,34}
\definecolor{Note}{RGB}{81,88,94}

\tikzset{
  tensor/.style={draw=Wgreen,line width=.9pt,decorate,
    decoration={snake,amplitude=1.05pt,segment length=5.8pt}},
  axion/.style={draw=CSred,line width=.85pt,dash pattern=on 3pt off 2.1pt},
  ymvertex/.style={circle,fill=YMblue,draw=YMblue,inner sep=0pt,minimum size=5.7pt},
  quarticvertex/.style={circle,fill=QuarticPink,draw=QuarticPink,
    inner sep=0pt,minimum size=5.7pt},
  csvertex/.style={rectangle,fill=CSred,draw=CSred,inner sep=0pt,minimum size=6.4pt},
  momentum/.style={font=\footnotesize,text=Ink,inner sep=1pt},
  momarrow/.style={draw=Ink,line width=.5pt,{Stealth[length=3.6pt,width=2.8pt]}-},
  weight/.style={font=\footnotesize,text=Ink,inner sep=1pt},
  derivative/.style={circle,draw=YMblue,fill=white,line width=.75pt,
    inner sep=0pt,minimum size=4.9pt}
}

\newcommand{\BackgroundCross}[2][Ink]{%
  \draw[#1,line width=.8pt,fill=white] (#2) circle[radius=.105];
  \draw[#1,line width=.8pt] ($(#2)+(-.074,-.074)$) -- ($(#2)+(.074,.074)$);
  \draw[#1,line width=.8pt] ($(#2)+(-.074,.074)$) -- ($(#2)+(.074,-.074)$);
}

% All arrows are momentum-flow arrows, not charge-flow arrows.
\newcommand{\MomentumK}{%
  \draw[momarrow] (1.09,.22) -- (.43,.22);
  \node[momentum,anchor=south] at (.76,.26) {$\mathbf k$};
}
\newcommand{\MomentumUpper}{%
  \draw[momarrow] (2.27,.92) -- (1.96,.61);
  \node[momentum,anchor=south] at (2.10,.95) {$\mathbf p$};
}
\newcommand{\MomentumLower}[1]{%
  \draw[momarrow] (2.27,-.92) -- (1.96,-.61);
  \node[momentum,anchor=north] at (2.10,-.95) {$#1$};
}

% Quadratic derivative kernel with normalized output-helicity projection.
\newcommand{\DiagramUW}{%
\begin{tikzpicture}[x=.91cm,y=.91cm,baseline=-.55ex]
  \coordinate (v) at (1.60,0);
  \draw[tensor] (0,0) -- (v);
  \draw[tensor] (v) -- (2.72,.85);
  \draw[tensor] (v) -- (2.72,-.85);
  \node[ymvertex] at (v) {};
  \node[derivative] at (1.63,.265) {};
  \MomentumK
  \draw[momarrow] (2.47,.81) -- (2.02,.47);
  \draw[momarrow] (2.47,-.81) -- (2.02,-.47);
  \node[momentum,anchor=south] at (2.21,.89) {$\mathbf p$};
  \node[momentum,anchor=north] at (2.21,-.89) {$\mathbf k-\mathbf p$};
  \node[weight,anchor=north east] at (1.48,-.15) {$g$};
\end{tikzpicture}%
}

% Cubic trace kernel, before subtraction of the internal trace contraction.
\newcommand{\DiagramVW}{%
\begin{tikzpicture}[x=.91cm,y=.91cm,baseline=-.55ex]
  \coordinate (v) at (1.60,0);
  \draw[tensor] (0,0) -- (v);
  \draw[tensor] (v) -- (2.48,.89);
  \draw[tensor] (v) -- (3.13,0);
  \draw[tensor] (v) -- (2.48,-.89);
  \node[quarticvertex] at (v) {};
  \MomentumK
  \MomentumUpper
  \MomentumLower{\mathbf k-\mathbf p-\mathbf q}
  \draw[momarrow] (2.96,.22) -- (2.38,.22);
  \node[momentum,anchor=south] at (2.67,.26) {$\mathbf q$};
  \node[weight,anchor=north east] at (1.48,-.15) {$g^2$};
\end{tikzpicture}%
}

% Trace-pair tadpole. The two remaining W legs include ONE stochastic
% contraction; its spectrum is absorbed in the complete graph notation.
\newcommand{\DiagramVTadpole}{%
\begin{tikzpicture}[x=.91cm,y=.91cm,baseline=-.55ex]
  \coordinate (v) at (1.25,0);
  \coordinate (lc) at (1.25,.49);
  \draw[tensor] (0,0) -- (v);
  \draw[tensor] (v) -- (2.50,0);
  \draw[tensor] (v) arc[start angle=-90,end angle=270,radius=.49];
  \node[quarticvertex] at (v) {};
  \draw[momarrow] (.65,.22) -- (.10,.22);
  \draw[momarrow] (2.28,.22) -- (1.90,.22);
  \draw[momarrow] ($(lc)+(60:.64)$)
    arc[start angle=60,end angle=0,radius=.64];
  \node[momentum,anchor=south] at (1.25,1.16) {$\mathbf p$};
  \node[momentum,anchor=south] at (.38,.26) {$\mathbf k$};
  \node[momentum,anchor=south] at (2.09,.26) {$\mathbf k$};
  \node[weight,anchor=north] at (1.25,-.16) {$g^2$};
\end{tikzpicture}%
}

% Quartic YM parent with a homogeneous zero-spatial-momentum Q insertion.
\newcommand{\DiagramZQ}{%
\begin{tikzpicture}[x=.91cm,y=.91cm,baseline=-.55ex]
  \coordinate (v) at (1.60,0);
  \coordinate (b) at (3.11,0);
  \draw[tensor] (0,0) -- (v);
  \draw[tensor] (v) -- (2.48,.89);
  \draw[tensor] (v) -- (2.48,-.89);
  \draw[tensor,draw=CSred] (v) -- (b);
  \node[quarticvertex] at (v) {};
  \BackgroundCross[CSred]{b}
  \MomentumK
  \MomentumUpper
  \MomentumLower{\mathbf k-\mathbf p}
  \node[momentum,text=CSred,anchor=west] at (3.31,0) {$Q\delta_i^{\,a}$};
  \node[weight,anchor=north east] at (1.48,-.15) {$g^2$};
\end{tikzpicture}%
}

% Effective CS interaction: the crossed dashed leg is the rolling axion.
% Its coupling normalization has been absorbed into phi.
\newcommand{\DiagramZphi}{%
\begin{tikzpicture}[x=.91cm,y=.91cm,baseline=-.55ex]
  \coordinate (v) at (1.60,0);
  \coordinate (a) at (3.11,0);
  \draw[tensor] (0,0) -- (v);
  \draw[tensor] (v) -- (2.48,.89);
  \draw[tensor] (v) -- (2.48,-.89);
  \draw[axion] (v) -- (a);
  \node[csvertex] at (v) {};
  \BackgroundCross[CSred]{a}
  \MomentumK
  \MomentumUpper
  \MomentumLower{\mathbf k-\mathbf p}
  \node[momentum,text=CSred,anchor=west] at (3.31,0) {$\dot\phi$};
  \node[weight,anchor=north east] at (1.48,-.15) {$g$};
\end{tikzpicture}%
}

\newcommand{\LegendYM}{\tikz[baseline=-.45ex]{\node[ymvertex] at (0,0) {};}}
\newcommand{\LegendQuartic}{\tikz[baseline=-.45ex]{\node[quarticvertex] at (0,0) {};}}
\newcommand{\LegendW}{\tikz[x=1cm,y=1cm,baseline=-.45ex]{\draw[tensor] (0,0)--(.55,0);}}
\newcommand{\LegendCS}{\tikz[baseline=-.45ex]{\node[csvertex] at (0,0) {};}}
\newcommand{\LegendDerivative}{\tikz[baseline=-.45ex]{\node[derivative] at (0,0) {};}}
\newcommand{\LegendQ}{\tikz[x=1cm,y=1cm,baseline=-.45ex]{\coordinate (b) at (.55,0);\draw[tensor,draw=CSred] (0,0)--(b);\BackgroundCross[CSred]{b}}}
\newcommand{\LegendAxion}{\tikz[x=1cm,y=1cm,baseline=-.45ex]{\coordinate (a) at (.50,0);\draw[axion] (0,0)--(a);\BackgroundCross[CSred]{a}}}

